Unbiased Active Inference for Classical Control

Active inference is a mathematical framework that originated in computational neuroscience. Recently, it has been demonstrated as a promising approach for constructing goal-driven behavior in robotics. Specifically, the active inference controller (AIC) has been successful on several continuous control and state-estimation tasks. Despite its relative success, some established design choices lead to a number of practical limitations for robot control. These include having a biased estimate of the state, and only an implicit model of control actions. In this paper, we highlight these limitations and propose an extended version of the unbiased active inference controller (u-AIC). The u-AIC maintains all the compelling benefits of the AIC and removes its limitations. Simulation results on a 2-DOF arm and experiments on a real 7-DOF manipulator show the improved performance of the u-AIC with respect to the standard AIC. The code can be found at https://github.com/cpezzato/unbiased_aic.

==> Tex/aic.tex <==
\section{The active inference controller}
Active Inference considers an agent in a dynamic environment that receives observations $\mathbf{y}$ about states $\mathbf{x}$. The agent then infers the posterior $p(\mathbf{x}|\mathbf{y})$ given a model of the agent's world. Instead of exactly calculating $p(\mathbf{x}|\mathbf{y})$, which could be computationally expensive, the agents approximates $p(\mathbf{x}|\mathbf{y})$  with a `variational distribution' $q(\mathbf{x})$ which we can define to have a standard form (Gaussian for instance). The goal is then to minimize the difference between the two distributions which is computed by the KL-divergence \cite{fox2012tutorial}: 

\begin{equation}
\begin{split}
    \label{eq:Kullback-leibler}
    KL(q(\mathbf{x})|| p(\mathbf{x}|\mathbf{y})) &= \int{q(\mathbf{x}) \ln{\frac{Q(\mathbf{x})}{p(\mathbf{x}, \mathbf{y})}}
    d\mathbf{x} + \ln p(\mathbf{y})}\\
    &= F + \ln p(\mathbf{y}).
\end{split}
\end{equation}

% \todo[inline]{$\mu$ is the mean of the distribution over states. However, if we move to formulation with explicit actions, we'll have a mean for the distribution over actions and also future states.}
The quantity $F$ is referred to as the (variational) free-energy -or Evidence lower bound- and minimizing F minimizes the KL-divergence. If we choose $q$($x$) to be a Gaussian distribution with mean $\pmb{\mu}$ and utilize the Laplace approximation \cite{friston2007variational}, the free-energy expression simplifies to:
\begin{equation}
\begin{split}
    \label{eq:laplace_F}
    F \approx &  -\ln p(\pmb{\mu}, \mathbf{y}) + C. %\\
    %&= - \ln p_t(y|\mu) - \ln p_t(\mu) + C
\end{split}
\end{equation}

Now the expression for variational free-energy is solely dependent on one parameter, $\pmb{\mu}$, which is referred to as the `belief state'. The objective is to find $\pmb{\mu}$ which minimizes $F$; this results in the agent finding the best estimate of its state.
 
 
% \subsection{Generalized motions}
% \label{sec:gen_motions}

Generalized motions (GM) \cite{friston2008hierarchical} are used to represent the (belief) states of a dynamical system, using increasingly higher order derivatives of the system state. This means that the n-dimensional state $\pmb{\mu}$ and its higher order derivatives are combined in $\pmb{\tilde{{\mu}}}$  ($\pmb{\tilde{\mu}} = [\pmb{\mu}, \pmb{\mu'} ...]$). The same can be done for the observations ($\mathbf{\tilde{y}} = [\mathbf{y}, \mathbf{y'}$ ...]).

For instance, in the context of a robotic manipulator, $\mathbf{y}$ represents the sensory observation of a joint position, while $\mathbf{y'}$ represents the joint's velocity observation. We consider GM up to the second order.

\subsection{Observation model and state transition model}
\label{sec:models_gen_and_sensory}

\textcolor{red}{I want to re-write this section and avoid using generalized motions too much.}
Taking generalized motions into account, the joint probability from (\cref{eq:laplace_F}) can be written as:

\begin{equation}
\begin{split}
    \label{eq:generative_model_p(mu,O)}
    p(\tilde{\mathbf{y}}, \pmb{\tilde{\mu}})
    &= p(\tilde{\mathbf{y}}| \pmb{\tilde{\mu}})p(\pmb{\tilde{\mu}}) = \underbrace{p(\mathbf{y}| \pmb{\mu})p(\mathbf{y'}| \pmb{\mu'})}_{\textrm{Observation model}}  \underbrace{p(\pmb{\mu'}| \pmb{\mu})p(\pmb{\mu''}| \pmb{\mu'})}_{\textrm{Transition model}},
\end{split}
\end{equation}
where $p(\mathbf{y}| \pmb{\mu})$ is the probability of receiving an observation $\mathbf{y}$ while in (belief) state $\pmb{\mu}$, and $p(\pmb{\mu'}| \pmb{\mu})$ is the state transition model (also referred to as the dynamic model or the generative model). The state transition model predicts the state evolution given the current state. These distributions are assumed Gaussian according to:
\begin{equation}
\begin{split}
    \label{eq:gaussian_model_for_gen_and_sen}
    p(\mathbf{y}| \pmb{\mu}) = \mathcal{N}(\mathbf{y}; g(\pmb{\mu}), \Sigma_y), & 
    \;\; p(\mathbf{y'}| \pmb{\mu'}) = \mathcal{N}(\mathbf{y}'; g'(\pmb{\mu'}), \Sigma_{y'}), \\
    p(\pmb{\mu'}| \pmb{\mu}) = \mathcal{N}(\pmb{\mu'}; f(\pmb{\mu}), \Sigma_{\mu}), &
   \;\; p(\pmb{\mu''}| \pmb{\mu'}) = \mathcal{N}(\pmb{\mu''}; f'(\pmb{\mu'}), \Sigma_{\mu'}),
\end{split}
\end{equation}
where the functions $g(\pmb{\mu})$ and $g'(\pmb{\mu'})$ represent a mapping between observations and states. For many application the state is directly observable, thus  $g(\pmb{\mu}) = \pmb{\mu}$ and $g'(\pmb{\mu'}) = \pmb{\mu'}$. 


The functions $f(\pmb{\mu})$ and $f(\pmb{\mu'})$ represent the evolution of the belief state over time. This encodes the agent's preference over future states (in this case the preferred future state is the reference trajectory, $\pmb{\mu_g}$). We assume: $f(\pmb{\mu}) = (\pmb{\mu_g} - \pmb{\mu})\tau^{-1}$ and $f'(\pmb{\mu'}) = (\pmb{\mu_g'} - \pmb{\mu}')\tau^{-1}$, where $\pmb{\mu_g}$ is the desired trajectory and $\tau$ is a temporal parameter. 

Given that all distributions are Gaussian, the expression for $F$ becomes a sum of quadratic terms and the natural logarithms:

\begin{equation}
\begin{split}
    \label{eq:laplace_F_final_vector}
    F  
    &=  \frac{1}{2}(\sum_{i} \pmb{\varepsilon}_{i}^\top \Sigma_{i}^{-1}\pmb{\varepsilon}_i + 
     \ln|\Sigma_i|)
    + C,
\end{split}
\end{equation}



\noindent where $i \in \left \{ \mathbf{y}, \mathbf{y}', \pmb{\mu}, \pmb{\mu}' \right \}$ and  $\pmb{\varepsilon_{\mu}} = \pmb{\mu'} - (\pmb{\mu_g} - \pmb{\mu})\tau^{-1}$, 
$\pmb{\varepsilon_{\mu'}} = \pmb{\mu''} - (\pmb{\mu_g'} - \pmb{\mu}')\tau^{-1}$, 
$\pmb{\varepsilon_{y}} = \mathbf{y} - \pmb{\mu}$ and  
$\pmb{\varepsilon_{y'}} = \mathbf{y'} - \pmb{\mu'}$ and $C$ refers to constant terms.



\subsection{Estimation and control}
\label{sec:F_and_minimization}

To achieve state estimation, we perform gradient descent on $F$ using the following update rules: 

\begin{equation}
    \label{eq:F_minimize_mu}
    \pmb{\dot{\tilde{\mu}}} = D\pmb{{\tilde{\mu}}} - \kappa_{\mu}\frac{\partial F}{\partial {\pmb{\tilde{\mu}}}},
\end{equation}


\noindent where $\kappa_{\mu}$ is the gradient descent step size and $D$ is a temporal derivative operator.

We thus perform one gradient descent step for each  iteration. To find suitable control actions, we would also use one-step gradient descent; however, the expression for $F$ does not include any actions and thus we resort to using the chain rule, assuming an implicit dependence between the actions performed by the agent and the measurements it acquires.

\begin{equation}
    \label{eq:F_minimize_a}
    \mathbf{\dot{u}} = - \kappa_{u}\frac{\partial F}{\partial \mathbf{u}}
    = - \kappa_{u} \frac{\partial F}{\partial \tilde{\mathbf{y}}}  \frac{\partial \tilde{\mathbf{y}}}{\partial \mathbf{u}},
\end{equation}

\noindent where $\kappa_{u}$ is the gradient descent step size. The term $\frac{\partial \tilde{\mathbf{y}}}{\partial \mathbf{u}}$ is assumed linear, and equal to the identity matrix (multiplied by a constant) similar to existing work ~\cite{pezzato2020novel, oliver2019active}.

Actions are then computed as:
\begin{equation}
    \label{eq:update_rules_a}
    \mathbf{\dot{u}} = -\kappa_{u}(\Sigma_{y}^{-1} (\mathbf{y} - \bm{\mu}) + \Sigma_{y'}^{-1} (\mathbf{y'} - \bm{\mu'})).
\end{equation}


\subsection{Simultaneous state-estimation and control}
Under this formulation, estimation and control are solved simultaneously and both processes are dependent. The observation terms (such as $\pmb{\varepsilon_{y}}$) refine the current belief $\pmb{\mu}$, whereas the reference terms $\pmb{\varepsilon_{\mu}}$ bias the estimated state towards the target $\pmb{\mu_g}$. In addition, if the parameters $\tau^{-1}$ and $\Sigma_{\mu}^{-1}$ are larger, the estimate $\pmb{\mu}$ is biased more towards the target $\pmb{\mu_g}$.


\textcolor{red}{We use mass-spring-damper, but I was thinking of using cruise control since its a much simpler system}

To illustrate this, consider the mass damper system given by the equation: $\ddot{x} = a(t) - k_1x - k_2\dot{x}$, where $x$ is the position of the mass, $a(t)$ the control action, $k_1$ the spring constant (set to $1 N/m$), $k_2$ the damper coefficient (set to $0.1 Ns/m$) and the system has unit mass. We simulated it with initial conditions $x(0) = -0.5m$, $\dot{x}(0) = -1 m/s$ and $a(t) = 0N$. Figure \ref{fig:estimation_only_differnt_delta_values} shows the results for the simulation when solving Equation \ref{eq:F_minimize_mu} for different values of $\tau^{-1}$.

Higher values of $\tau^{-1}$ give more bias toward the target. For $\tau^{-1} = 8$ (green line), the estimate is close to the target (black dashed line) and far away from the actual position (blue dashed line) as opposed to setting $\tau^{-1} = 0.1$ (red line). If $\tau^{-1} \rightarrow  0$, the estimation step reduces to a pure estimator, which would follow the trajectory without any bias toward the target.

The controller steers the system based on the observation error terms ($\pmb{\varepsilon_{y}}$ and $\pmb{\varepsilon_{y'}}$). Since larger values of $\tau^{-1}$ move the estimate more towards the target, the difference given by $\mathbf{y} - \pmb{\mu}$ is larger and thus the controller is more aggressive. An illustration for the control behaviour given different values of $\tau^{-1}$ is shown in Figure \ref{fig:control_different_delta_values}. 

